Bayesian Model Calibration for Extrapolative Prediction via Gibbs Posteriors

The current standard Bayesian approach to model calibration, which assigns a Gaussian process prior to the discrepancy term, often suffers from issues of unidentifiability and computational complexity and instability. When the goal is to quantify uncertainty in physical parameters for extrapolative prediction, then there is no need to perform inference on the discrepancy term. With this in mind, we introduce Gibbs posteriors as an alternative Bayesian method for model calibration, which updates the prior with a loss function connecting the data to the parameter. The target of inference is the physical parameter value which minimizes the expected loss. We propose to tune the loss scale of the Gibbs posterior to maintain nominal frequentist coverage under assumptions of the form of model discrepancy, and present a bootstrap implementation for approximating coverage rates. Our approach is highly modular, allowing an analyst to easily encode a wide variety of such assumptions. Furthermore, we provide a principled method of combining posteriors calculated from data subsets. We apply our methods to data from an experiment measuring the material properties of tantalum.

==> figures/Table_SimResults1.tex <==
% latex table generated in R 3.5.2 by xtable 1.8-3 package
% Tue Feb 26 13:27:13 2019
\begin{table}[ht]
\centering
\begin{tabular}{l|rr|rr}
  & \multicolumn{2}{c|}{Fixed} & \multicolumn{2}{c}{Estimated} \\ & E(w) & Coverage & E(w) & Coverage \\ 
  \hline
Non-parametric bootstrap & 0.14 & 0.76 & 0.15 & 0.79 \\ 
  Parametric bootstrap & 0.07 & 0.88 & 0.07 & 0.79 \\ 
  Effective sample size & 0.05 & 0.93 & 0.05 & 0.86 \\ 
  \end{tabular}
\caption{Frequentist coverage for high autocorrelation time.  
       Nominal coverage is 90\%.\label{tab:simresults1}} 
\end{table}


==> input/Data-Application-OLD.tex <==


\section{Application to dynamic material properties}
\label{sec:dataapp}

Dynamic material models describe how materials behave at extreme
conditions of high pressures and temperatures.  % The experiments
% considered in this example reached peak pressures between 70–240 GPa,
% which are of the order of the pressure in the Earth’s inner core.
To calibrate these material models, we couple computational
predictions of velocity over time with experimental measurements.  In
this application, our goal is to calibrate parameters of the tantalum
equation of state, namely the bulk modulus $B_0$ and its pressure
derivative $B_0'$ based on the model form of \cite{vinet1989}.

Here we overview the structure of the problem; details are further
discussed in \cite{brown2018}. We analyze the same data here to
illustrate how our method works.  We have data from 9 different
experimental measurements.  In the experiments, a pulsed power driver
delivers massive electrical currents over short time scales through an
aluminum panel, resulting in a time-dependent stress wave (impulse)
propagating through the tantalum samples and then through transparent
lithium fluoride windows (Figure \ref{fig:exp}, left panel).  The
output of interest in the velocity over time at the tantalum-lithium
fluoride interface (Figure \ref{fig:exp}, right
panel).  % The experimentally measured velocities
% were then compared against computational predictions.
Inputs to the computer model predictions include the material
properties of interest for calibration and other experimental
uncertainties, including: uncertainty in the boundary condition, which
specifies the impulse imposed on the material sample; the thicknesses
of the tantalum and aluminum samples; and the initial tantalum
density.

\begin{figure}[!ht]
  \centering
\includegraphics[width=.37\textwidth]{figures/Figure2_Configuration-eps-converted-to.pdf}
\includegraphics[width=.5\textwidth]{figures/Figure3_ExpVels-eps-converted-to.pdf}
\caption{\textit{Left}: Experimental configuration.  A time-dependent
  magnetic field (boundary condition) results in a time-dependent
  stress wave propagating through the system; the experimental output
  is the velocity measured at the interface between the tantalum
  sample and lithium-flouride window. \textit{Right}: Nine different
  velocity curves from experiments with different thicknesses and/or
  boundary conditions.}
\label{fig:exp}
\end{figure}


Because the same tantalum plate was used to generate samples across
all experiments, the material properties and density of tantalum do
not vary between experiments.  Differences between the experiments
occur due to different thicknesses of the tantalum samples and
different boundary conditions.  A single experiment produces a
functional output (a velocity curve measured over time) which can be
sampled at a high rate.  While there is a small amount of measurement
uncertainty in velocity at each time point, smoothing this curve can
essentially eliminate this measurement noise at each time point, such
that the experimental outputs can be considered smooth with no
measurement noise.

In this application, model discrepancy arises because there is no
combination of model inputs for which the computationally predicted
velocity curve can exactly match the experimental measurement (Figure
\ref{fig:expdisc}).  Whether this arises due to experimental
uncertainties that distort the velocity curve or due to actual
computational model error does not matter here for the mathematical
formulation of discrepancy. Furthermore, since the goal is quantifying
uncertainty in these physical parameters for the sake of extrapolative
prediction (i.e., prediction in contexts outside these experiments),
our method of Gibbs posteriors for model calibration is appropriate to
use here.  Since we have nine different experiments, with separate
functional discrepancies expected for each, it is also convenient to
calibrate each one separately and combine their respective posteriors
using our ensemble approach.


\begin{figure}[!ht]
\centering
\includegraphics[width=.45\textwidth]{figures/Figure_CISPoster_Discrepancy.png}
\caption{Example of model discrepancy in a single experiment.}
\label{fig:expdisc}
\end{figure}


For the $j$\textsuperscript{th} experiment, we consider modeling the
output as $y(x_j) = \eta(x_j; \theta) + \delta(x_j) $, where
$\eta(x_{j}; \theta)$ is the computational model prediction of
velocity at $n_j=n=100$ time points $x_j$ with input values of the
calibration parameters $\theta$, and $\delta(x_j)$ is the discrepancy
between the model prediction and experimental measurement.  Failing to
account for model discrepancy would essentially result in the
uncertainty of the calibration parameters decreasing arbitrarily with
the number of points sampled from the functional output.

In the original analysis of these data, \cite{brown2018} apply both a
standard KOH model and a power-likelihood approach to account for
model discrepancy. Equivalently, we may say they implemented a Gibbs
posterior with the loss function being the Gaussian negative
log-likelihood,
\begin{align}\label{eq:loss-brown}
  l(y_j, \theta, \sigma) =
  \frac{n}{2} \log(2\pi\sigma^2) +
  \sum_{i=1}^{n} \frac{[y(x_{ji}) - \eta(x_{ji}; \theta)]^2}{2\sigma^2}.
\end{align}  
Although we previously made the comment that we can effectively assume
no error in the experimental measurements, the $\sigma^2$ parameter is
included in this loss function to quantify the scale of the
discrepancy, which is also potentially useful to compare across
experiments. To select the loss scales $w_j$ for the Gibbs posteriors
$p_w(\theta \mid y_j) \propto \exp(-w_j l(y_j, \theta, \sigma))
\pi(\theta)$, they first obtain a point estimate for the parameters
giving the best fitting output to the data,
$(\hat \theta_j, \hat \sigma_j) = \arg \min_{\theta, \sigma} l(y_j,
\theta, \sigma)$ and then select $w_{j}$ based on the effective sample
size (ESS) $n_{ej}$ of the empirical discrepancy
$\hat \delta(x_j) = y(x_j) - \eta(x_j; \hat \theta_j)$, so that
$\hat w_j^\text{ESS} = n_{ej} / n$.  To compute the full posterior for
$\theta$, they use the joint loss function, assuming independence
between experiments,
$p(\theta \mid y) \propto \prod_{j=1}^9 \exp(- \hat w^\text{ESS}_j
l(y_j, \theta, \sigma)) \pi(\theta)$. They conclude that the Gibbs
posterior generates more computationally stable results that are
consistent with prior knowledge about the material properties.

% \sw{Lauren: previously in this section you mention that we can ignore
%   error variance, but that is contradicted in this paragraph and in
%   the fact that the loss function \eqref{eq:loss-brown} has a $\sigma$
%   component.  So this section should be edited for clarity.  Also,
%   this paragraph feels extraneous anyway so maybe we should just cut
%   it. } Note that the loss function in Eq. \eqref{eq:loss-brown} can
% be extended to other likelihoods.  Further, the error-variance model
% can be extended to allow for residual overdispersion, i.e.,
% $\sigma(x) = \phi \sigma_m(x)$, where $\phi$ accounts for
% overdispersion in residuals beyond measurement uncertainty - a type of
% model misspecification).

Here we reanalyze the data making two changes.  First, we implement
the parametric bootstrap procedure of
Section~\ref{sec:parametric-bootstrap} to tune the choice of loss
scales $w_j$ for each experiment.  We use these to obtain posteriors
for each experiment independently.  Then, we use the WASP method of
ensemble calibration in Section~\ref{sec:ensemble-calibration} to
combine the posteriors for each experiment into one consensus
posterior.  For the sake of comparison, we will also calculate the
WASP consensus posterior using posteriors formed using loss scales
from the ESS method.  We use the same loss function
\eqref{eq:loss-brown} for the Gibbs posterior, and assign the weakly
informative priors $B_0 \sim \mathcal{U}(155, 215)$,
$B'_0 \sim \mathcal{U}(2.9, 4.9)$ and
$\sigma^2 \sim \mathcal{IG}(0.01, 0.01)$.


We use the empirical Bayes variant of the parametric bootstrap
procedure, assuming that the discrepancy follows a mean-0 GP with
squared exponential covariance kernel (for simplicity we drop the $j$
subscript and explain the procedure for one experiment).  We first
calculate the empirical discrepancy term $\hat \delta(x)$ exactly as
done by \cite{brown2018}.  Then we estimate the hyperparameters for
the Gaussian process using maximum marginal likelihood on
$\hat \delta$ % and the estimated residual variance
% $\hat{\sigma}^2$ using maximum marginal likelihood on this empirical
% discrepancy,
to calculate an estimate of it covariance matrix $\hat \Sigma$.

One bootstrap dataset is calculated as follows.  First, take a draw
from the prior for $\theta$, $\theta^{(b)} \sim \pi(\theta)$, and
sample a bootstrap discrepancy term using
$\delta^{(b)} \sim \N(0, \hat
\Sigma)$. % , and a bootstrap sample for the
% error term using $\epsilon^{(b)} \sim \N(0, \hat{\sigma}^2\I)$
The bootstrap dataset is calculated by
$y^{(b)}(x)= \eta(x; \theta^{(b)}) + \delta^{(b)}(x)$.  We then form
equal-tailed Gibbs posterior credible intervals using $y^{(b)}$ for a
defined grid of possible loss scale values $\{w\}$, and check whether
these intervals bracket $\theta^{(b)}$.  Following this procedure for
$b=1,\ldots,B = 100$ gives a Monte Carlo estimate of frequentist
coverage for the Gibbs posterior with these values of $\{w\}$.  Since
we are interested in two parameters, for one value of $w$ we average
the coverage rate between the two parameters. We considered 35 values
of $w$ on a log-scale for each experiment, and then fit an
interpolating spline to estimate coverage as a function of $w$, with
the inverse standard error as weights for fitting the spline, and use
a root finding algorithm to find which $w$ gives the nominal
frequentist coverage of $1-\alpha=0.9$.

Figure~\ref{fig:cover-plot-avg} shows the results of the parametric
bootstrap procedure for choosing the Gibbs posterior loss scales
$w_{j}$ for each experiment $j=1,\ldots, 9$, and compares them to
those calculated from the residual ESS.  At times the two differ
widely, suggesting that the loss scales from ESS method could result
in poor frequentist metrics. In addition, the loss scales from the
parametric bootstrap tend to be closer to one another than those from
ESS.  

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.85\textwidth]{figures/cover-plot-avg.pdf}
  \caption{\label{fig:cover-plot-avg} Results of parametric bootstrap
    procedure for choosing the loss function selecting scaling factor.
    The estimated coverage on the $y$-axis is an average of the
    coverage between the two parameters, $B_0$ and $B_0'$.  }
\end{figure}

Finally, Figure~\ref{fig:gibbs-combined} compares the consensus
posteriors resulting from the two scaling factor selection methods for
the two parameters of interest.  Because we combine inference across
distinct experiments, we scale the consensus by a factor of $1/9$, as
explained in Section~\ref{sec:comb-subs-post}. Both consensus
posteriors have similar marginal variances for the parameters, likely
because the scaling factors from the two methods are, on average,
similar in magnitude.  However, since each experiment is weighted
differently between the two methods, the means are quite far apart.
The online supplement gives the loss scales and subset posteriors for
each experiment for both methods.

The resulting posteriors for both methods differ from those from the
original results from; the posterior means for $B_0$ are slightly
higher than those in the previous analysis, while the posterior means
for $B'_0$ is slightly lower, and the posterior variance is also lower
than originally reported.  We believe these disparities to arise from
using a different emulator for the computer model for
$\eta(x; \theta)$.  We used an emulator based on multivariate adaptive
regression splines (MARS) \citep{friedman1991}, rather than Gaussian
process regression used by the original paper.


\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.65\textwidth]{figures/gibbs-posterior-final-combined.pdf}
  \caption{\label{fig:gibbs-combined} Combined posteriors for
    $(B_0, B'_0)$ using the WASP ensemble calibration method, for both
    methods of loss scale selection.  }
\end{figure}

\begin{figure}[!ht]
  \centering
  \includegraphics[width=0.95\textwidth]{figures/gibbs-posterior-bp0-all.pdf}
  \caption{\label{fig:gibbs-combined2} Combined posteriors for
    $(B_0, B'_0)$ using the WASP ensemble calibration method, for both
    methods of loss scale selection.  }
\end{figure}



%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Draft"
%%% End:



==> input/Ensemble_old.tex <==

\section{Ensemble calibration}
\label{sec:ensemble-calibration}

In some calibration problems, it may be advantageous to divide the
data into subsets, calibrate on the subsets, and then combine
inferences across them.  We consider two primary motivations for
calibrating in subsets: (i) it can be more computationally efficient,
particularly when datasets are large and/or calibration parameters
vary over the model space $x \in \X$; and (ii) when the discrepancy is
non-stationary over $\X$, updating the loss separately for different
subsets of $\X$ will often be simpler than trying to specify a joint
loss and discrepancy prior over all of $\X$.  For example, in the
material model calibration problem described in
Section~\ref{sec:dataapp}, material properties can be calibrated
separately for each experiment and then combined over experiments to
produce a global estimate.  Discrepancy may differ by experiment; by
estimating $\theta$ separately for each one, we do not have to
incorporate the changing magnitude of the discrepancy into the loss
function, and we can gauge how much information each experiment
provides about $\theta$ in the presence of discrepancy.

We refer to the idea of calibrating in subsets as ``ensemble
calibration.''  Section \ref{sec:choosew} considered choosing a single $w$ for the entire dataset. % The coverage calibration methods in Section
% \ref{sec:choosew} selected a single $w$ for the entire dataset.
In ensemble calibration, model misspecification is considered for
subsets of the data.  The data are subdivided over $\X$ into $K$
subsets and each subset receives its own loss scale, so the full
posterior is
 \begin{align}
  p(\theta \mid y) \propto \prod_{k=1}^K
  \exp(-w_k(y_k \mid \theta))\pi(\theta), \label{eq:jointpost}
\end{align}
with the methods in Sections \ref{sec:choosew} and
\ref{sec:parametric-bootstrap} used to select loss scales $w_k$ for the
different subsets.

Directly updating the model in Eq.~\eqref{eq:jointpost} is
disadvantageous.  \cite{gunawan2017bayesian} show that directly
calibrating this joint posterior of the weighted subsets results in
consistent estimates of $\theta$, but uncertainty in $\theta$ is
underestimated. % (they propose a data
% augmentation approach to posterior inference as an alternative to the
% joint posterior.  are calibrated separated for each subset)
An alternative solution is to calibrate each subset separately and
obtain a posterior for each one:
\begin{eqnarray} p(\theta \mid y_k) \propto \exp(-w_k
l(y_k \mid \theta))\pi(\theta), \quad k=1,\ldots,K. \label{eq:obayes2}
\end{eqnarray} 
The posteriors $p(\theta \mid y_k)$ can then be combined \textit{post
  hoc} to produce an overall estimate of the calibration parameters.
This approach has computational advantages, in that calibrating each
subset is simpler than the joint calibration problem.  Further, the
ensemble calibration approach is advantageous because we get model
diagnostics for free.  That is, allowing $\theta$ to vary over $x$
could help diagnose areas of the model space $x$ where model
discrepancy could substantively change the calibration parameters.
Calibrating subsets separately provides information about how
calibration parameter estimates vary across the input space, which
informs how discrepancy impacts the calibration parameter estimates.

Ensemble calibration is closely related to distributed Bayesian
analysis, where data is divided into subsamples for subset inference
\citep{scott2016bayes}. The resulting subset posteriors are combined
into a consensus posterior distribution approximating the full data
posterior. Similarly, ensemble calibration entails solving the
calibration problem on subsets of the data and combining the results.

\subsection{Combining subset posteriors}
\label{sec:comb-subs-post}
We apply the recently developed method of Wasserstein scalable
posteriors (WASP) to combine subset posteriors
\citep{pmlr-v38-srivastava15}. WASP divides the data into $K$ subsets,
finding posteriors $\Pi_k$ for each subset $k=1,\ldots,K$; then,
subset posteriors are combined into a consensus posterior $\bar{\Pi}$
by calculating an approximate Wasserstein barycenter or an ``average''
(with respect to Wasserstein distance) of the subset posterior
distributions.  As long as the number of subsets $K$ is not growing
too quickly with the sample size $n$, WASP achieves almost optimal
convergence to the true parameter, $\theta$, and WASP produces
estimates that asymptotically converge to the full data posterior,
even for many models with independent and non-identically distributed
observations \citep{2015arXiv150805880S}.  The consensus mean is an
inverse covariance-weighted average of the subset means, and an
iterative algorithm, described in the supplement, is used to calculate
the consensus covariance matrix. There is a question of scaling the
consensus posterior. It may be scaled by $1/K$ to model the covariance
of parameters \emph{across} experiments; otherwise, we effective model
the covariance of parameters \emph{within} an experiment, which is
more appropriate when calibrating only a single experiment that is
partitioned into subsets.

Combining subset posteriors using the Wasserstein metric has several
advantages.  The Wasserstein metric encodes geometric information
about the distribution and the sample space. For example, the
Wasserstein barycenter between distributions of the same
location-scale family will also be in the same location-scale
family. This does not hold for Euclidean barycenters of distributions
in the same location-scale family.  These factors make the WASP
approach more flexible in the setting of ensemble calibration. There
is no need to down-weight priors. The method can also handle
deviations from Gaussianity and different specifications of loss
function.

We outline our algorithmic process for combining subset
posteriors and give additional detail in the online supplement; for
general background in this area, see \cite{Villani2003, villani2006,
  gouicloubes2017, aguehcarlier2011, alvarezestebanetal2016}.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Draft"
%%% End:


==> input/Ensemble_old2.tex <==

\section{Ensemble calibration}
\label{sec:ensemble-calibration}

In some calibration problems, it may be advantageous to divide the
data into subsets, calibrate on the subsets, and then combine
inferences across them.  We consider two primary motivations for
calibrating in subsets: (i) it can be more computationally efficient,
particularly when datasets are large and/or calibration parameters
vary over the model space $x \in \X$; and (ii) when the discrepancy is
non-stationary over $\X$, updating the loss separately for different
subsets of $\X$ will often be simpler than trying to specify a joint
loss and discrepancy prior over all of $\X$.  For example, in the
material model calibration problem described in
Section~\ref{sec:dataapp}, material properties can be calibrated
separately for each experiment and then combined over experiments to
produce a global estimate.  Discrepancy may differ by experiment; by
estimating $\theta$ separately for each one, we do not have to
incorporate the changing magnitude of the discrepancy into the loss
function, and we can gauge how much information each experiment
provides about $\theta$ in the presence of discrepancy.

We refer to the idea of calibrating in subsets as ``ensemble
calibration.''  Section \ref{sec:choosew} considered choosing a single
$w$ for the entire
dataset. % The coverage calibration methods in Section
% \ref{sec:choosew} selected a single $w$ for the entire dataset.
In ensemble calibration, model misspecification is considered for
subsets of the data.  The data are subdivided over $\X$ into $K$
subsets and each subset receives its own loss scale, so the full
posterior is
 \begin{align}
  p(\theta \mid y) \propto \prod_{k=1}^K
  \exp(-w_k l(y_k \mid \theta))\pi(\theta), \label{eq:jointpost}
\end{align}
with the methods in Sections \ref{sec:choosew} and
\ref{sec:parametric-bootstrap} used to select loss scales $w_k$ for the
different subsets.

Directly updating the model in Eq.~\eqref{eq:jointpost} is
disadvantageous.  \cite{gunawan2017bayesian} show that directly
calibrating this joint posterior of the weighted subsets results in
consistent estimates of $\theta$, but uncertainty in $\theta$ is
underestimated. % (they propose a data
% augmentation approach to posterior inference as an alternative to the
% joint posterior.  are calibrated separated for each subset)
An alternative solution is to calibrate each subset separately and
obtain a posterior for each one:
\begin{eqnarray} p(\theta \mid y_k) \propto \exp(-w_k
l(y_k \mid \theta))\pi(\theta), \quad k=1,\ldots,K. \label{eq:obayes2}
\end{eqnarray} 
The posteriors $p(\theta \mid y_k)$ can then be combined \textit{post
  hoc} to produce an overall estimate of the calibration parameters.
This approach has computational advantages, in that calibrating each
subset is simpler than the joint calibration problem.  Further, the
ensemble calibration approach is advantageous because we get model
diagnostics for free.  That is, allowing $\theta$ to vary over $x$
could help diagnose areas of the model space $x$ where model
discrepancy could substantively change the calibration parameters.
Calibrating subsets separately provides information about how
calibration parameter estimates vary across the input space, which
informs how discrepancy impacts the calibration parameter estimates.

Ensemble calibration is closely related to distributed Bayesian
analysis, where data is divided into subsamples for subset inference
\citep{scott2016bayes}. The resulting subset posteriors are combined
into a consensus posterior distribution approximating the full data
posterior. Similarly, ensemble calibration entails solving the
calibration problem on subsets of the data and combining the results.

\subsection{Combining subset posteriors}
\label{sec:comb-subs-post}
We apply the recently developed method of Wasserstein scalable
posteriors (WASP) to combine subset posteriors
\citep{pmlr-v38-srivastava15}. WASP divides the data into $K$ subsets,
finding posteriors $\Pi_k$ for each subset $k=1,\ldots,K$; then,
subset posteriors are combined into a consensus posterior $\bar{\Pi}$
by calculating an approximate Wasserstein barycenter or an ``average''
(with respect to Wasserstein distance) of the subset posterior
distributions.  As long as the number of subsets $K$ is not growing
too quickly with the sample size $n$, WASP achieves almost optimal
convergence to the true parameter, $\theta$, and WASP produces
estimates that asymptotically converge to the full data posterior,
even for many models with independent and non-identically distributed
observations \citep{2015arXiv150805880S}.

Here we use the WASP framework to provide a coherent framework for
combining individually calibrated experiments into a consensus
posterior. For the consensus mean we use an inverse
covariance-weighted average of the subset means. While the Wasserstein
barycenter mean is the unweighted average of individual means, we
think a covariance-weighted average is better here for two reasons.
First in our framework the covariance of each experiment is not only
another parameter but also a quantification of uncertainty about the
parameter of interest. Second, when normal likelihoods are used, this
method provides an exact consensus posterior mean
\cite{scott2016bayes}, if we factor individual loss scales.

Finally, we note that computing the consensus mean in this manner has
no effect on the consensus covariance computation. An iterative
algorithm, described in the supplement, is used to calculate the
consensus covariance matrix. There is a question of scaling the
consensus posterior. In their original paper, Srivastava et al. use
the ``stochastic approximation trick''; each subset likelihood is
raised to the power of $K$. This is forces the consensus posterior to
reflect that we have $nK$ as opposed $n$ total data points. This
models the covariance of parameters \emph{across} all experiments;
each experiment provides a noisy estimate of $p(\theta)$ and
information across experiments is pooled, providing greater
power. Otherwise, we effectively model the covariance of parameters
\emph{within} an individual experiment, the covariance of an
``average'' experiment. This approach may be more appropriate when
subset posteriors are calibrating across large, varying portions of
$\X$ and when discrepancy is non-stationary.

Combining subset posteriors using the Wasserstein metric has several
advantages.  The Wasserstein metric encodes geometric information
about the distribution and the sample space. For example, the
Wasserstein barycenter between distributions of the same
location-scale family will also be in the same location-scale
family. This does not hold for Euclidean barycenters of distributions
in the same location-scale family.  These factors make the WASP
approach more flexible in the setting of ensemble calibration. There
is no need to down-weight priors, as with other methods, potentially losing conjugacy. The method can also handle
deviations from Gaussianity and different specifications of loss
function.

We outline our algorithmic process for combining subset
posteriors and give additional detail in the online supplement; for
general background in this area, see \cite{Villani2003, villani2006,
  gouicloubes2017, aguehcarlier2011, alvarezestebanetal2016}.




%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Draft"
%%% End:


==> input/Motivating-Example.tex <==


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../Draft"
%%% End:


==> input/_region_.tex <==
\message{ !name(Introduction.tex)}
\message{ !name(Introduction.tex) !offset(-2) }

\section{Introduction}

Model calibration is the process of learning about model inputs by
coupling experimental data with computational simulation outputs,
essentially solving an inverse problem for a deterministic computer
model.  Model calibration can serve two distinct purposes in computer
modeling: interpolative prediction and extrapolative prediction.  In
interpolative prediction, the model parameters are tuned such that the
model can accurately predict throughout the design space \textit{where
data have been collected}.  In extrapolative prediction, the
calibrated model results are applied to predict in a space
\textit{where no data have been collected and the model cannot be
directly validated}.  Extrapolative prediction is common in many
engineering applications, as the computer modeling exercise is often
intended to compensate for gaps in data.  Examples of extrapolative
prediction include: calibrating subsystem models to roll-up results
into overall system predictions \citep{li2016role}, using calibration
to estimate parameters with scientific meaning
\citep{brown2018,brynjarsdottir2014learning}, and using models to
predict to spaces where data cannot be collected
\citep{ling2014selection}.

Calibration is often a poorly identified problem, where multiple
inputs produce equally valid solutions.  Bayesian inference has been
used extensively in model calibration to avoid optimization challenges
under poorly identified parameters.  Specifically, the
\cite{kennedy2001bayesian} Bayesian model calibration framework
(abbreviated as the KOH model) is the most popular statistical
approach for calibration, as this model allows for calibration under
different uncertainties, including input parameter uncertainty,
measurement uncertainty in the experimental data, and model-form
error.  This paper is concerned with the latter uncertainty,
model-form error.

Models are inherently approximations of reality and typically contain
error; thus, model calibration procedures must accommodate for model
discrepancy (also called model misspecification in the statistics
literature) to obtain valid estimates and uncertainties on calibrated
input parameters.  The question of whether a `true' value of a model
inputs exists in reality is a philosphically debatable question,
because there is no ground truth in a computer simulation.  We take a
pragmatic view here, in that a true calibration parameter exists
insofar as it is informative to extrapolative prediction; we refer to
such calibration parameters as `physical parameters' to reflect the
notion that these parameters represent some true physical value that
informs extrapolative prediction, following
\citep{brynjarsdottir2014learning}.

When model inputs have physical interpretations, model discrepancy
must be carefully considered for valid physical parameter estimation
and uncertainty quantification (UQ).  For instance,
\cite{brynjarsdottir2014learning} illustrate that the KOH model
results in biased parameter estimates in the presence of systematic
model discrepancy and that the only way to reduce this bias using the
KOH model is to \textit{a priori} know the form of the discrepancy.
Challenges associated with physical parameter calibration under model
misspecification are well-documented \citep{arendt2012improving,
  arendt2012quantification, brynjarsdottir2014learning,
  arendt2016preposterior, tuo2016theoretical}, but few solutions exist
beyond the standard \cite{kennedy2001bayesian} treatment of model
discrepancy.  \lh{added the following sentences per spencer's
  comments:} A common thread across all calibration under model
discrepancy methodologies is that the analyst must make assumptions
about the form of the model discrepancy in order to obtain accurate
calibration parameter estimates.  For instance, the KOH model assumes
that model discrepancy can be represented as a Gaussian process;
further, inferences about $\theta$ under KOH are generally only
correct when the Gaussian procss is mean 0 and independent of the
model inputs.  \cite{brynjarsdottir2014learning} place stronger prior
information on the Gaussian process under a non-mean 0 discrepancy to
improve inferences based on knowledge of the form of the discrepancy.

The goal of this report is to introduce an alternative to the KOH
model for accommodating model discrepancy, namely power-likelihood
models.  While this approach does not solve the physical parameter
identifiability problem, it does provide an alternative modeling
framework to KOH that allows the analyst to learn additional
information about the model discrepancy, utilizing \textit{a priori}
knowledge of how the model is wrong when possible.  The
power-likelihood framework emphasizes the need for distinct treatments
of calibration for interpolative versus extrapolative prediction,
analogous to predictive versus explanatory modeling in statistics
\citep{shmueli2010explain}.  For extrapolative prediction,
alternatives to KOH are lacking but needed.


\section{Motivating example}

\section{Review of KOH and model discrepancy}

The most commonly used calibration model, referred to as the Kennedy
and O'Hagan (KOH) model, is \citep{kennedy2001bayesian}:
		\begin{eqnarray} y(x)& =& \eta(x, \theta) +
\delta_j(x) + \epsilon(x) \nonumber \\ \delta &\sim& N(\mu_{\delta},
\Sigma^{\delta}) \nonumber \\ \epsilon &\sim& N(0,\sigma)
		\label{eq:koh}
		\end{eqnarray} where $x \in \mathcal{X}$ are known
control inputs that are controlled by design (e.g. experimental test
conditions, time) and vary over input space $\mathcal{X}$; $\theta \in
\Theta$ are calibration parameters; $\eta$ is the true value of the
outcome as a function of $x$ and $\theta$; $\epsilon$ is random
measurement error in the outcome, and $\delta$ is a Gaussian process
model discrepancy term, accounting for inaccuracies in the computer
model predictions.
                
                % For our purposes, the difference between $\gamma$ %
and $\theta$ is that $\theta$ is used for % extrapolative prediction,
whereas $\gamma$ is not % (i.e., $\gamma$ is a nuisance parameter).
		
The KOH model allows for model misspecification through incorporation
of the Gaussian process discrepancy term.  However, it is well known
that including a Gaussian process to `account for model discrepancy'
is insufficient, because $\theta$ and $\delta$ are not jointly
identifiable. The calibration parameters $\theta$ are only guaranteed
to converge to their true physical values when there is no discrepancy
$\delta = 0$ or when the discrepancy is mean 0 over $x$ and
independent of $\theta$.  Calibration parameters should not be
expected to have physical interpretations under the KOH model
\citep{loeppky2006computer,arendt2012improving,brynjarsdottir2014learning}.
The non-identifiability of the discrepancy function is similar to the
problem of `spatial confounding' in the spatial statistics literature
\citep{reich2006effects, hodges2010adding, paciorek2010importance} and
differential measurement error in the statistical measurement error
literature; it is generally not possible to learn a systematic,
unobserved model bias from the observed data.

More recent work \citep{tuo2016theoretical} shows that KOH calibration
is not L2-consistent and calibration parameter inferences depend on
the model discrepancy prior.  \cite{plumlee2017bayesian} proposes
using a prior on the discrepancy that is orthogonal to the computer
model gradient to produce calibration results that are consistent with
the desired loss function, similar to projected kernel calibration
proposed in \citep{tuo2017adjustments}.  \lh{added the following per
spencer's comments} Given the lack of consistency, another trend in
the calibration literature is to view calibration as an optimization
problem \citep{tuo2015efficient, gramacy2015calibrating,
wong2017frequentist}, with the optimization problem commonly defined
as minimization of the L-2 norm over $x$.  Specifically,
\begin{eqnarray} \text{argmin}_{\theta \in \Theta} \int_{x \in
\mathcal{X}} \left[\eta(\theta, x) - y(x)\right]^2dF(x) \label{eq:l2}
\end{eqnarray} While viewing calibration as optimization (as in
Equation \ref{eq:l2}) simplifies the definition of the `best-estimate'
of $\theta$ relative to KOH, there is still a need to measure
uncertainty in the estimated calibration parameters.



\message{ !name(Introduction.tex) !offset(-151) }

